Topic Discovery and Classification for Responsible Generative AI Adaptation in Higher Education

As generative artificial intelligence (GenAI) becomes increasingly capable of delivering personalized learning experiences and real-time feedback, a growing number of students are incorporating these tools into their academic workflows. They use GenAI to clarify concepts, solve complex problems, and, in some cases, complete assignments by copying and pasting model-generated contents. While GenAI has the potential to enhance learning experience, it also raises concerns around misinformation, hallucinated outputs, and its potential to undermine critical thinking and problem-solving skills. In response, many universities, colleges, departments, and instructors have begun to develop and adopt policies to guide responsible integration of GenAI into learning environments. However, these policies vary widely across institutions and contexts, and their evolving nature often leaves students uncertain about expectations and best practices. To address this challenge, the authors designed and implemented an automated system for discovering and categorizing AI-related policies found in course syllabi and institutional policy websites. The system combines unsupervised topic modeling techniques to identify key policy themes with large language models (LLMs) to classify the level of GenAI allowance and other requirements in policy texts. The developed application achieved a coherence score of 0.73 for topic discovery. In addition, GPT-4.0-based classification of policy categories achieved precision between 0.92 and 0.97, and recall between 0.85 and 0.97 across eight identified topics. By providing structured and interpretable policy information, this tool promotes the safe, equitable, and pedagogically aligned use of GenAI technologies in education. Furthermore, the system can be integrated into educational technology platforms to help students understand and comply with relevant guidelines.

==> related_works.tex <==
\section{Related Works}
To the extent of the research conducted, no standardized criteria categorization methods exist for GenAI academic policies. The adoption of a clause, guideline document, or academic policy addressing GenAI varies amongst higher education institutions in the United States (U.S.). Within individual institutions, guidelines and policies are subject to vary at the institution, department, and course level. Any policy established is subject to change at any of the aforementioned levels. Academic integrity policies for ethical GenAI usage—as with any form of academic engagement—in education must be explicitly established:

% \begin{displayquote}
% “[A]mbiguity of expectations and a disproportionate focus on student action, but not on that of staff, results in an environment where different, and often conflicting, academic integrity practices may operate in parallel leading to even greater inconsistency and procedural unfairness.” \cite{assesment_and_evaluation_in_higher_education}
% \end{displayquote}

% To be effective, GenAI academic policies must be revised at a rate proportional to the speed of technological changes \cite{school_of_information_student_research_journal}. Consequently, guardrails for GenAI’s academic usage must be proportionally receptive to changes in academic integrity policies

% The current (as of July 2024) literature adopts syllabi as a tangible benchmark to quantify the integration of GenAI into higher education systems \cite{creative_education}. A non-GenAI-assisted review finds that GenAI academic policies fall under the following categories: “AI for cheating; AI as legitimate support; an equity, diversity, and inclusion lens into AI; and emerging recommendations to tackle AI implications in higher education” \cite{canadian_perspectives_on_academic_integrity}. However, the literature adopts syllabi evaluation using artificial intelligence (AI) as both possible and accepted for quality control assurance \cite{association_for_computing_machinery}. The statistically significant present-day level of artificial intelligence (AI) adoption in post-higher-education professions is sufficient to prompt the incorporation of AI usage into preparatory curriculums \cite{hct}. However, GenAI academic integrity policies—when included—in syllabi are inconsistent across assignment types within the same classroom. R1 (very high research activity) higher education institutions in the U.S. orient their GenAI guidelines and policies to most frequently address ethical concerns of its knowledge production and its usage in writing-based works. GenAI policies for STEM-related academic works are statistically more vague and infrequently addressed than writing-related works \cite{mcdonald2024generative}. Vagueness between usages of GenAI in the classroom jeopardizes students’ academic integrity by putting them at greater risk of committing academic fraud.

In the current literature, there exists both a gap and a need to automatically classify GenAI policy criteria and their allowance based on policy documents. This section provides a call to action for the discovery of a classification framework for GenAI academic policies in higher education.

